Contrastive Explanations That Anticipate Human Misconceptions Can Improve Human Decision-Making Skills

People's decision-making abilities often fail to improve or may even erode when they rely on AI for decision-support, even when the AI provides informative explanations. We argue this is partly because people intuitively seek contrastive explanations, which clarify the difference between the AI's decision and their own reasoning, while most AI systems offer "unilateral" explanations that justify the AI's decision but do not account for users' thinking. To align human-AI knowledge on decision tasks, we introduce a framework for generating human-centered contrastive explanations that explain the difference between AI's choice and a predicted, likely human choice about the same task. Results from a large-scale experiment (N = 628) demonstrate that contrastive explanations significantly enhance users' independent decision-making skills compared to unilateral explanations, without sacrificing decision accuracy. Amid rising deskilling concerns, our research demonstrates that incorporating human reasoning into AI design can foster human skill development.

==> sections/7-exploratory-analysis.tex <==
\section{Exploratory Analysis}

% How do different designs affect people's weighing of different dimensions

% aot_group impacts post performance for contrastive predicted and contrastive random, but not unilateral, contrastive update and no AI


%Our results (Figure~\ref{fig:results-learning}) showed that participants learned significantly more with contrastive explanations with predicted or inputted foil compared to receiving no AI support (lending support to \textbf{H-L1}). Importantly, and as expected (\textbf{H-L2a}), contrastive explanations with a predicted foil led to significantly greater learning compared to unilateral explanations. However, the difference in learning between contrastive explanations with an inputted foil and unilateral explanations was not significant, not supporting \textbf{H-L2b}.
%Moreover, also as hypothesized (\textbf{H-A1a}), the improvement in learning for contrastive predicted was achieved without sacrificing accuracy: participants completing the task with contrastive explanations with predicted or inputted foul were as accurate as their counterparts who received unilateral explanations (Figure~\ref{fig:results-accuracy}). Additionally, participants in the contrastive explanations with predicted foil condition reported significantly greater perceived autonomy (but not significantly different competence and relatedness to AI) during the task compared to those in the unilateral condition, providing partial support for \textbf{HS-1}. On the 

==> sections/results-w-variables.tex <==
\section{Results}

\subsection{Main results}


\subsubsection{Human Learning}


Main results for learning are depicted in Figure~\ref{fig:results-learning}. We report adjusted p-values, corrected with Holm-Bonferroni to account for multiple comparisons.
As hypothesized (\textbf{H-L1a} \& \textbf{H-L1b}), participants experienced statistically significantly greater learning in the \textit{contrastive predicted} ($M = \getvar{lr-mean-cp}$, $F_{\getvar{lr-n-df-cp-noAI}, \getvar{lr-d-df-cp-noAI}} = \getvar{lr-f-stat-cp-noAI}$, $p = \getvar{lr-p-cp-noAI}$, $d = \getvar{lr-eff-cp-noAI} \ [\getvar{lr-efflo-cp-noAI}, \getvar{lr-effup-cp-noAI}]$) and \textit{contrastive after} ($M = \getvar{lr-mean-ca}$, $F_{\getvar{lr-n-df-ca-noAI}, \getvar{lr-d-df-ca-noAI}} = \getvar{lr-f-stat-ca-noAI}$, $p = \getvar{lr-p-ca-noAI}$, $d = \getvar{lr-eff-ca-noAI} \ [\getvar{lr-efflo-ca-noAI}, \getvar{lr-effup-ca-noAI}]$) conditions compared to participants in the no AI condition ($M = \getvar{lr-mean-noAI}$).

Participants in the \textit{contrastive random} condition also showed significantly higher gains than those in the no AI condition ($M = \getvar{lr-mean-cr}$, $F_{\getvar{lr-n-df-cr-noAI}, \getvar{lr-d-df-cr-noAI}} = \getvar{lr-f-stat-cr-noAI}$, $p = \getvar{lr-p-cr-noAI}$, $d = \getvar{lr-eff-cr-noAI} \ [\getvar{lr-efflo-cr-noAI}, \getvar{lr-effup-cr-noAI}]$). Conversely, participants in the \textit{unilateral} condition did not signficantly improve their learnring compared to \textit{no AI} ($M = \getvar{lr-mean-un}$, $F_{\getvar{lr-n-df-un-noAI}, \getvar{lr-d-df-un-noAI}} = \getvar{lr-f-stat-un-noAI}$, $p = \getvar{lr-p-un-noAI}$, $d = \getvar{lr-eff-un-noAI} \ [\getvar{lr-efflo-un-noAI}, \getvar{lr-effup-un-noAI}]$).

Comparing contrastive conditions with sensible foil to unilateral explanations, as hypothesized (\textbf{H-L2a}), participants in the \textit{contrastive predicted} condition ($M = \getvar{lr-mean-cp}$) learned statistically significantly more than participants in the \textit{unilateral} condition ($M = \getvar{lr-mean-un}$, $F_{\getvar{lr-n-df-cp-un}, \getvar{lr-d-df-cp-un}} = \getvar{lr-f-stat-cp-un}$, $p = \getvar{lr-p-cp-un}$, $d = \getvar{lr-eff-cp-un} \ [\getvar{lr-efflo-cp-un}, \getvar{lr-effup-cp-un}]$). However, the difference between \textit{contrastive after} ($M = \getvar{lr-mean-ca}$) and \textit{unilateral} explanations was not significant ($F_{\getvar{lr-n-df-ca-un}, \getvar{lr-d-df-ca-un}} = \getvar{lr-f-stat-ca-un}$, $p = \getvar{lr-p-ca-un}$, $d = \getvar{lr-eff-ca-un} \ [\getvar{lr-efflo-ca-un}, \getvar{lr-effup-ca-un}]$), not lending support to \textbf{H-L2b}.

Within the contrastive conditions, participants in the \textit{contrastive predicted} condition demonstrated greater learning ($M = \getvar{lr-mean-cp}$) compared to those in the \textit{contrastive random} condition ($M = \getvar{lr-mean-cr}$). However, this difference was only marginally significant ($F_{\getvar{lr-n-df-cp-cr}, \getvar{lr-d-df-cp-cr}} = \getvar{lr-f-stat-cp-cr}$, $p = \getvar{lr-p-cp-cr}$, $d = \getvar{lr-eff-cp-cr} \ [\getvar{lr-efflo-cp-cr}, \getvar{lr-effup-cp-cr}]$), offering partial support for hypothesis \textbf{H-L3}. Addressing research question \textbf{RQ-L1}, the \textit{contrastive predicted} condition did not result in significantly different learning compared to the \textit{contrastive after} condition ($M = \getvar{lr-mean-ca}$, $F_{\getvar{lr-n-df-cp-ca}, \getvar{lr-d-df-cp-ca}} = \getvar{lr-f-stat-cp-ca}$, $p = \getvar{lr-p-cp-ca}$, $d = \getvar{lr-eff-cp-ca} \ [\getvar{lr-efflo-cp-ca}, \getvar{lr-effup-cp-ca}]$).



\begin{figure}
     \centering
     \includegraphics[width=0.4\textwidth]{figures/overreliance.pdf}
     \label{fig:overreliance-by-condition}
     % \end{subfigure}
     % \begin{subfigure}{0.45\textwidth}
     % \includegraphics[width=\textwidth]{figures/overreliance_vs_learning.pdf}
     % \caption{Overreliance vs. learning}
     % \label{fig:overreliance-vs-learning}
     % \end{subfigure}
     \caption{Overreliance across conditions. Error bars represent one standard error.}
\end{figure}


\subsubsection{Accuracy and Overreliance}

\begin{figure*}
     \centering
     \includegraphics[width=0.9\textwidth]{figures/subjective_by_condition.pdf}
     
     \caption{Subjective results. Error bars represent one standard error.}
     \label{fig:results-subjective}
\end{figure*}

Figure~\ref{fig:results-accuracy} summarizes results of human accuracy on the decision task with different conditions. 
As hypothesized (\textbf{H-A1a} \& \textbf{H-A1b}), the accuracy of participants in the \textit{contrastive predicted} ($M = \getvar{acc-mean-cp}$, $F_{\getvar{acc-n-df-cp-un}, \getvar{acc-d-df-cp-un}} = \getvar{acc-f-stat-cp-un}$, $p = \getvar{acc-p-cp-un}$, $d = \getvar{acc-eff-cp-un} \ [\getvar{acc-efflo-cp-un}, \getvar{acc-effup-cp-un}]$) and \textit{contrastive after} ($M = \getvar{acc-mean-ca}$, $F_{\getvar{acc-n-df-ca-un}, \getvar{acc-d-df-ca-un}} = \getvar{acc-f-stat-ca-un}$, $p = \getvar{acc-p-ca-un}$, $d = \getvar{acc-eff-ca-un} \ [\getvar{acc-efflo-ca-un}, \getvar{acc-effup-ca-un}]$) conditions was not significantly different from that of participants in the \textit{unilateral} condition ($M = \getvar{acc-mean-un}$).

While participants improved their performance on the task significantly on average when they received AI support ($M = 0.56$) compared to receiving no AI support ($M = 0.31$, $F_{1, 627} = 195.32$, $p \ll 0.0001$), their performance also significantly degraded when AI suggestions were suboptimal ($M = 0.14$) compared to receiving no support ($M = 0.29$, $F_{1, 627} = 36.34$, $p \ll 0.0001$). Note that the different means for no AI support ($M = 0.31$, $M = 0.29$) in this analysis occur because we split the performance of participants in the no AI condition based on whether AI, if provided, would have been correct or incorrect, to allow a fairer comparison with other conditions that received incorrect suggestions for only a subset of questions. 

In situations when AI provided a suboptimal recommendation, participants in the \textit{contrastive predicted} ($M = \getvar{ov-mean-cp}$, $F_{\getvar{ov-n-df-cp-un}, \getvar{ov-d-df-cp-un}} = \getvar{ov-f-stat-cp-un}$, $p = \getvar{ov-p-cp-un}$, $d = \getvar{ov-eff-cp-un} \ [\getvar{ov-efflo-cp-un}, \getvar{ov-effup-cp-un}]$) and \textit{contrastive random} ($M = \getvar{ov-mean-cr}$, $F_{\getvar{ov-n-df-cr-un}, \getvar{ov-d-df-cr-un}} = \getvar{ov-f-stat-cr-un}$, $p = \getvar{ov-p-cr-un}$, $d = \getvar{ov-eff-cr-un} \ [\getvar{ov-efflo-cr-un}, \getvar{ov-effup-cr-un}]$) exhibited similar overreliance as those in the unilateral condition ($M = \getvar{ov-mean-un}$), addressing \textbf{RQ-A1}. %When the AI provided incorrect suggestions, participants in the \textit{contrastive predicted} [[add chi-square]] and \textit{contrastive random} [[add chi-square]]conditions were significantly more likely to choose the presented foil compared to those in the \textit{unilateral} condition.

Similarly, presenting contrastive explanations immediately (\textit{contrastive predicted}), resulted in similar overreliance ($M = \getvar{ov-mean-cp}$)  compared to presenting contrastive explanations after a decision was made (\textit{contrastive after}) ($M = \getvar{ov-mean-ca}$, $F_{\getvar{ov-n-df-cp-ca}, \getvar{ov-d-df-cp-ca}} = \getvar{ov-f-stat-cp-ca}$, $p = \getvar{ov-p-cp-ca}$, $d = \getvar{ov-eff-cp-ca} \ [\getvar{ov-efflo-cp-ca}, \getvar{ov-effup-cp-ca}]$). 

%% results about AOT and NFC x contrastive explanations



\subsubsection{Subjective Experience}

Subjective results are summarized in Figure~\ref{fig:results-subjective}.

%%Post-hoc Holm

%competence: {noAI, contrastive_update} < {unilateral, contrastive, contrastive_random}

Condition was a significant predictor of perceived competence ($F_{\getvar{competence-n-df-all}, \getvar{competence-d-df-all}}=\getvar{competence-f-stat-all}$, $p \ll \getvar{competence-p-all}$). A Holm-Bonferroni corrected post-hoc test revealed that participants in the \emph{contrastive predicted}, \emph{contrastive random}, and \emph{unilateral} conditions reported significantly higher competence compared to those in the \emph{contrastive after} and \emph{no AI} conditions.


%choice: {contrastive_update, unilateral} < {contrastive, contrastive_random, noAI}

Perceived autonomy (\emph{i.e.}, choice)  was also significantly predicted by condition ($F_{\getvar{choice-n-df-all}, \getvar{choice-d-df-all}}=\getvar{choice-f-stat-all}$, $p \ll \getvar{choice-p-all}$).
A Holm-Bonferroni corrected post-hoc test revealed that participants in the \emph{contrastive predicted}, \emph{contrastive random}, and \emph{no AI} conditions perceived significantly higher autonomy compared to those in the \emph{unilateral} and \emph{contrastive after} conditions.

%relatedness -- not including AI: {contrastive_update} < {contrastive, unilateral, contrastive_random}

Condition was also a significant predictor of relatedness to AI (computed only for conditions involving AI) ($F_{\getvar{relatedness-n-df-all}, \getvar{relatedness-d-df-all}}=\getvar{relatedness-f-stat-all}$, $p \ll \getvar{relatedness-p-all}$), with a Holm-Bonferroni post-hoc test revealing that participants in the \emph{contrastive after} condition felt significantly less related to the AI compared to those in other AI conditions.

%interest not significantly different
Task enjoyment/interest was not significantly predicted by condition ($F_{\getvar{interest-n-df-all}, \getvar{interest-d-df-all}}=\getvar{interest-f-stat-all}$, $p = n.s.$) and neither was mental demand ($F_{\getvar{demand-n-df-all}, \getvar{demand-d-df-all}}=\getvar{demand-f-stat-all}$, $p = \getvar{demand-p-all}$).
%self_efficacy: {noAI -- 1, contrastive_update--12, unilateral--23, contrastive_random -- 3, contrastive  -- 3}

Across measures, the subjective results support \textbf{H-S2}, showing that contrastive explanations with a predicted foil led to significantly higher perceptions of competence, autonomy, and relatedness to the AI compared to the contrastive after condition. Additionally, our findings partially support \textbf{H-S1}: while contrastive explanations with a predicted foil significantly increased perceived autonomy compared to unilateral explanations, no significant differences were observed for competence and relatedness to the AI. 

%\subsection{Additional analyses}


\subsubsection {Subjective vs. objective measures}


\begin{figure*}
     \centering
     \includegraphics[width=0.7\textwidth]{figures/objective_vs_subjective_all_final.pdf}
     
     \caption{Relationship between subjective experience vs. objective outcomes. R indicates Pearson's $r$. Only conditions with AI support are included in the analysis.}
     \label{fig:subjective-vs-objective}
\end{figure*}

Figure~\ref{fig:subjective-vs-objective} shows the relationship between subjective experience and objective outcomes across conditions with AI support (\em i.e. \em, no AI condition was not included in the analysis). Our analysis revealed that there was no correlation between actual learning and competence, autonomy, or mental demand and that actual learning was very weakly inversely correlated with relatedness to AI ($r = - 0.08, p = 0.06$) and task enjoyment ($r = - 0.09, p = 0.04$).
Accuracy was significantly positively correlated with relatedness to AI ($r = 0.26, p \ll 0.0001$), a construct that included questions about trust in AI too, and it was significantly negatively correlated with perceived autonomy ($r = -0.15, p = 0.0003$). Similarly, overreliance was significantly positively correlated with relatedness to AI ($r = 0.22, p \ll 0.0001$), and significantly negatively correlated with perceived autonomy ($r = -0.15, p = 0.0006$). In addition, overreliance was significantly positively correlated with task enjoyment ($r = 0.1, p = 0.02$).

%\subsubsection{Overreliance vs. learning}

%We investigated the relationship between overreliance and learning, contributing evidence to the ongoing conversation in AI-assisted decision-making~\cite{buccinca2024towards}. Scholars have suggested that both constructs are rooted in cognitive engagement, as learning sciences have shown a strong link between learning and engagement. The AI-assisted decision-making literature has further proposed that increased cognitive engagement with AI could reduce overreliance~\cite{bucinca2021trust, gajos2022people}. Similar to ~\citet{buccinca2024towards}, we found a very weak and non-significant, partial correlation (controlling for performance on pre-test questions) between overreliance and learning ($r = -0.06 [-0.13, 0.02]$, $p = 0.13$, with 95\% CI based on 1000 bootstrap samples), indicating that factors beyond cognitive engagement may be influencing overreliance.



%AOT significanlty positively correlated with performance on intervention questions and increased learning. NFC a weaker marginally predictor of performance on intervention questions, and not a predictor of learning.
%NFC signficantly positively correlated with higher intrinsic motivation --- competence, autonomy, and relatedness to AI.

\subsection {Audit for intervention-generated inequalities}
%may change to intervention generated inequalities

\begin{figure*}
     \centering
     \begin{subfigure}{0.48\textwidth}
     \includegraphics[width=\textwidth]{figures/learning_by_NFC.pdf}
     \caption{Need for Cognition (NFC)}
     \label{fig:learning-NFC}
     \end{subfigure}
     \begin{subfigure}{0.48\textwidth}
     \includegraphics[width=\textwidth]{figures/learning_by_AOT.pdf}
     \caption{Actively Open-minded Thinking (AOT)}
     \label{fig:learning-AOT}
     \end{subfigure}
     \caption{Auditing for intervention generated inequalities: Learning (marginal means) for different individual differences. Error bars represent one standard error. Significance levels after Holm-Bonferroni correction are indicated by: * p < 0.05.}
\end{figure*}

Intervention-generated inequalities occur when an intervention, while beneficial on average, disproportionately benefits some groups over others~\cite{lorenc2013types}. Disaggregating results by relevant demographics or variables can help uncover these disparities. Informed by prior research in AI-assisted decision-making~\cite{bucinca2021trust, gajos2022people}, we conduct a self-audit and examine whether contrastive explanations, introduced as interventions to enhance human decision-making skills, benefit different groups equally.

Previous studies have shown that individual differences in information processing can significantly impact the effectiveness of AI support and interventions, particularly for cognitively demanding outcomes like learning. One individual difference that may affect the effectiveness of our interventions is Need for Cognition (NFC), a stable trait that reflects an individual's motivation to engage in deep thinking and information processing~\cite{cacioppo1982need}. NFC has been consistently identified as a predictor of performance in cognitive tasks such as problem-solving and decision-making~\cite{cacioppo96:dispositional}. In the context of AI-assisted decision-making, NFC has been found to influence whether cognitive forcing reduces overreliance on AI~\cite{buccinca2021trust} and how effectively individuals learn from AI assistance~\cite{gajos2022people, buccinca2024towards}.

Another important individual difference that we reasoned would be particularly relevant for interventions that require consideration of multiple viewpoints is Actively Open-Minded Thinking (AOT). People high in AOT are more likely to critically evaluate new evidence, weigh it against their existing beliefs, take sufficient time to solve problems, and carefully consider others' opinions when forming their own~\cite{baron1993teach, haran2013role}. We investigate whether individuals with varying levels of AOT benefit differently from contrastive explanations, which provide alternative ``viewpoints'' for consideration.

Figures~\ref{fig:learning-NFC} and ~\ref{fig:learning-AOT} depict results disaggregated by NFC and AOT. We did not find any significant differences among the effectiveness of (any) contrastive explanations for people with different levels of NFC (for detailed ananlyses see Appendix, Table~\ref{tab:nfc-results}). 
However, our findings reveal a notable contrast in the AOT groups: participants with high AOT benefited significantly more from the \emph{contrastive predicted} condition ($M=0.52$) compared to those with low AOT ($M=0.42$; $F_{1, 122} = 6.67$, $p = 0.01$, $d = 0.47$ [$0.11$, $0.84$]). Similarly, the \emph{contrastive random} condition was more effective for individuals with high AOT ($M=0.46$) than for those with low AOT ($M=0.42$; $F_{1, 142} = 3.77$, $p = 0.05$, $d = 0.34$ [$-0.01$, $0.68$]). See Table~\ref{tab:aot-results} for non-significant conditions.
These findings uncover AOT as a relevant individual difference to consider in AI-assisted decision-making and reveal that contrastive explanations may unevenly impact individuals, offering greater advantages to those with higher AOT.


%Across conditions, AOT level was a significant predictor of learning. Individuals high in AOT ($M = 0.43$), low AOT ($M = 0.38$, $F_{2, 622} = 9.10$, $p = .0002$). And it was a signifcant predictor of performance on intervention questions. Individuals high in AOT ($M = 0.43$), low AOT ($M = 0.38$, $F_{2, 622} = 9.10$, $p = .0002$)


%On the other hand, NFC group was not a predictor of learning. Individuals high in NFC ($M = 0.42$), low NFC ($M = 0.40$, $F_{2, 622} = 1.08$, $p = n.s.$). It was a predictor of overall performance, but not overreliance ($F_{2, 622} = 1.48$, $p = n.s.$).
